Test-Time Adaptation For Speech Enhancement Via Mask Polarization

Adapting speech enhancement (SE) models to unseen environments is crucial for practical deployments, yet test-time adaptation (TTA) for SE remains largely under-explored due to a lack of understanding of how SE models degrade under domain shifts. We observe that mask-based SE models lose confidence under domain shifts, with predicted masks becoming flattened and losing decisive speech preservation and noise suppression. Based on this insight, we propose mask polarization (MPol), a lightweight TTA method that restores mask bimodality through distribution comparison using the Wasserstein distance. MPol requires no additional parameters beyond the trained model, making it suitable for resource-constrained edge deployments. Experimental results across diverse domain shifts and architectures demonstrate that MPol achieves very consistent gains that are competitive with significantly more complex approaches.

==> fig/data/comp/dist_ideal.tex <==
\begin{tikzpicture}
	\begin{axis}[
			axis x line=bottom,
			axis y line=center,
			yticklabel={\empty},
			ytick=\empty,
			xtick=\empty,
			xticklabel={\empty},
			ymin=0.0, ymax=16000,
			xmin=-0.2, xmax=1.3,
			width=9em, height=8em,
		]

		\addplot[apfelgruen, fill=apfelgruen!50]
		table [x=x, y=y]
			{fig/data/comp/ideal.txt};

	\end{axis}
\end{tikzpicture}


==> fig/data/comp/dist_pre.tex <==
\begin{tikzpicture}
	\begin{axis}[
			axis x line=bottom,
			axis y line=center,
			yticklabel={\empty},
			ytick=\empty,
			xtick=\empty,
			xticklabel={\empty},
			ymin=0.0, ymax=16000,
			xmin=-0.2, xmax=1.3,
			width=9em, height=8em,
		]


		\addplot[mittelblau, fill=mittelblau, name path=f, fill opacity=0.5]
		table [x=x, y=y]
			{fig/data/comp/pre.txt};


	\end{axis}
\end{tikzpicture}


==> fig/data/comp/dist_source.tex <==
\begin{tikzpicture}
	\begin{axis}[
			axis x line=bottom,
			axis y line=center,
			yticklabel={\empty},
			ytick=\empty,
			xtick=\empty,
			xticklabel={\empty},
			ymin=0.0, ymax=16000,
			xmin=-0.2, xmax=1.3,
			width=9em, height=8em,
		]


		\addplot[orange, fill=orange, name path=f, fill opacity=0.5]
		table [x=x, y=y]
			{fig/data/comp/source.txt};

		% \path[name path=axis] (axis cs:-0.1,0) -- (axis cs:1.5,0);



	\end{axis}
\end{tikzpicture}


==> fig/data/comp/dist_ss.tex <==
\begin{tikzpicture}
	\begin{axis}[
			axis x line=bottom,
			axis y line=center,
			yticklabel={\empty},
			ytick=\empty,
			xtick=\empty,
			xticklabel={\empty},
			ymin=0.0, ymax=16000,
			xmin=-0.2, xmax=1.3,
			width=9em, height=8em,
		]


		\addplot[moosgruen, fill=moosgruen!50]
		table [x=x, y=y]
			{fig/data/comp/ss.txt};

	\end{axis}
\end{tikzpicture}


==> fig/data/dist_src.tex <==
\begin{tikzpicture}
	\begin{axis}[
			axis x line=bottom,
			axis y line=left,
			yticklabel={\empty},
			ytick=\empty,
			xtick=\empty,
			xticklabel={\empty},
			ybar,
			ymin=0.0, ymax=21000,
			xmin=-0.3, xmax=9,
            bar width=0.525em,
            width=10em, height=10em,
		]

        \addplot[mittelblau, fill=mittelblau!50]
		coordinates {
				(0, 19371)
				(1, 7387)
				(2, 5500)
				(3, 4128)
				(4, 3999)
				(5, 3808)
				(6, 3618)
				(7, 3673)
				(8, 8179)
			};

	\end{axis}
\end{tikzpicture}


==> fig/data/dist_targ.tex <==
\begin{tikzpicture}
	\begin{axis}[
			axis x line=bottom,
			axis y line=left,
			yticklabel={\empty},
			ytick=\empty,
			xtick=\empty,
			xticklabel={\empty},
			ybar,
			ymin=0.0, ymax=21000,
			xmin=-0.3, xmax=9,
            bar width=0.525em,
            width=10em, height=10em,
		]

        \addplot[orange, fill=orange!50]
		coordinates {
				(0, 2094)
				(1, 4209)
				(2, 8777)
				(3, 10146)
				(4, 9463)
				(5, 6731)
				(6, 5858)
				(7, 6347)
				(8, 8362)
			};

	\end{axis}
\end{tikzpicture}

